Distilling Text LMs into Speech-to-Speech LMs by Matching Internal Text Predictions

Text language models (LMs) acquire broad linguistic and factual capabilities through large-scale pretraining, while comparable capabilities remain difficult to learn from speech alone. Recent work has shown that knowledge distillation from pretrained text LMs offers a promising way to transfer their linguistic and factual capabilities to speech models. However, existing distillation approaches have largely focused on speech-input, text-output models. This idea has yet to be explored for {\it speech-to-speech} models, which operate on both speech input and speech output. In this work we introduce a speech-to-speech pretraining method that creates an internal text interface for knowledge transfer while preserving the speech-only input and output. The model first consumes speech context without its transcription, switches to text prediction, and then uses the predicted text to lead future speech generation word by word. It also provides an interface for knowledge distillation: the internal text predictions can be directly distilled from the base text LM. To the best of our knowledge, this is the first application of text LM distillation to a speech-to-speech LM. Under matched training conditions, the proposed sequence construction substantially improves the generative perplexity of spoken continuations over speech-only and interleaved speech-text models, approaching the performance of a text-leading inner-monologue model with external ASR prompt transcription. More importantly, distillation improves factual performance under both text and speech evaluation, indicating better retention of knowledge from the base text language model.

==> backup.tex <==
\section{Method}
\subsection{Speech representations and loss}
We use Flow-SLM's ~\cite{chou2023toward} objective and speech representaions. Specifically, for speech input, we use the prequantized mimi representations~\cite{defossez2024moshi}. For the speech output, we firstly predict the future $4$ semantic tokens (i.e. first level of RVQ tokens in Mimi tokenizer), and a following conditional flow-matching objective is used to predict the pre-quantized features. We use x-prediction objective~\cite{} like in~\cite{modgap}. 

\subsection{Sequence construction}
We show the sequence example in Fig.~\ref{fig:arch}.
We firstly obtain the word-level alignment using Whisper~\cite{}. We sample a word boundary as switch point. Before the speech point, we don't apply loss to the output. After the switch point, we construct the sequence by firstly predicting the word in text tokens, and then followed by its corresponding speech. To be able to switch modality during inference, we generate text end-of-word (\textit{<t-eow>}) special token after finishing the text word. After the speech word, we similarly generate a speech end of word (\textit{<s-eow>}) special token. For the speech end of word, we reuse the first semantic token head (the one corresponding to $t+1$ position), to train to predict the speech end of word. At each step, only text output head or speech related output head will be trained. 

\subsection{Distillation}
As shown in Fig\ref{fig:arch}, we distill from text teacher model during the steps that predictiing the next text tokens. We use the backbone model (the initialized text LM), as the teacher model. 

\subsection{Inference}
We treat prompt as the speech context, and insert a switch token right after the prompt. For generation based task, we generate text tokens until text end of word token. Then we generate speech until speech end of word becomes the top-1 rank in the first semantic token head. We do so until the model generate text eos token, then we will finish at the subsequent speech end of word. 

For likelihood based inference (scoring the continuation), we only score the text tokens. 


[explain the sequence]
[maybe no need for flow]
[evaluation]

==> external_model_hyperparameters.tex <==
% Requires \usepackage{booktabs,tabularx}
% External inference settings, checkpoints, and comparative StoryCloze protocol.
% Sources and inherited-filter audit: training_hyperparameters.sources.json
\begin{table*}[t]
\centering
\small
\begingroup
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\textwidth}{@{}p{0.25\textwidth}p{0.16\textwidth}p{0.10\textwidth}p{0.10\textwidth}X@{}}
\toprule
\textbf{External model} & \textbf{Temperature} & \textbf{Top-$p$} & \textbf{Top-$k$} & \textbf{Generation limit / key setting} \\
\midrule
SpiritLM Base / Expressive (7B) & 0.8 & 0.95 & 50 & 300 new speech-model tokens or 50 new text tokens; speaker ID 2; output modality forced \\
MiMo-Audio-7B-Base & 0.6 global; 0.9 local & 0.95 both & 50 both & $\lceil25s/g\rceil+1$ global steps, with duration budget $s$ and speech-frame group size $g=4$ \\
SLAM-Large & 0.8 & 1.0 & 25 & 150 new speech-unit tokens \\
Llama-Mimi-1.3B / 8B & 0.8 & 0.9 & 30 & 1,500 new tokens for current Emilia/Gemini-Emo; 1,024 total tokens in the saved Known-1000 zero-VAD runs \\
Qwen3-0.6B / 1.7B text backbones & 0.8 & 0.95 & 50 & 64 new text tokens for Known-1000; EOS-prefix reference for the plotted 0.6B comparison \\
\bottomrule
\end{tabularx}
\endgroup
\caption{Evaluation hyperparameters of the external baselines, used with their released weights and no task-specific fine-tuning. All listed generation paths enable sampling. Inherited filters are resolved from the local checkpoint configurations and evaluation-library defaults: top-$k=50$ for SpiritLM and Qwen, top-$p=1.0$ for SLAM (no nucleus truncation), and top-$p=0.9$ for Llama-Mimi. These are the inference settings used in our comparisons, not the models' original pretraining hyperparameters.}
\label{tab:external-decoding-hyperparameters}
\vspace{2pt}
\begin{minipage}{\textwidth}
\footnotesize
Top-$k$ and top-$p$ filtering are applied sequentially: top-$k$ first, followed by nucleus filtering on the renormalized remaining distribution. Both filters are active for SpiritLM, MiMo (global and local), Llama-Mimi, and the Qwen text backbones. SLAM uses top-$k$ only because $p=1.0$.
Generation uses five samples per prompt. Saved speech continuations are capped at 10 s for Known-1000 and 20 s for Emilia/Gemini-Emo; native termination and model-token limits can end them sooner. Duration caps do not apply to text output. Current external Emilia/Gemini-Emo runs use full-utterance encoding with floor prefix selection, joint prompt/continuation synthesis, no silence suppression, and no minimum speech duration. Saved Known-1000 speech inputs use end VAD and frame padding: 40 ms for SpiritLM/MiMo/SLAM and 80 ms for Llama-Mimi. The older Llama-Mimi Known-1000 token limit includes prompt tokens.
\end{minipage}
\end{table*}

\begin{table*}[t]
\centering
\small
\begin{tabularx}{\textwidth}{@{}p{0.29\textwidth}X@{}}
\toprule
\textbf{External model} & \textbf{Checkpoint identifier} \\
\midrule
SpiritLM Base / Expressive & \texttt{spirit-lm-base-7b} / \texttt{spirit-lm-expressive-7b} \\
MiMo-Audio-7B-Base & \texttt{XiaomiMiMo/MiMo-Audio-7B-Base} \\
SLAM-Large & \texttt{slprl/slam\_large} \\
Llama-Mimi-1.3B & \texttt{llm-jp/Llama-Mimi-1.3B} \\
Llama-Mimi-8B & \texttt{llm-jp/Llama-Mimi-8B} \\
Text backbone references & \texttt{Qwen/Qwen3-0.6B-Base}; \texttt{Qwen/Qwen3-1.7B-Base} \\
\bottomrule
\end{tabularx}
\caption{External checkpoint identities. Exact available revisions and local checkpoint provenance are retained in the evaluation contracts.}
\label{tab:external-checkpoints}
\end{table*}

% Likelihood evaluation is separate from sampled continuation generation.
\begin{table*}[t]
\centering
\small
\begin{tabularx}{\textwidth}{@{}p{0.26\textwidth}XX@{}}
\toprule
\textbf{StoryCloze setting} & \textbf{Our models} & \textbf{SpiritLM Base / Expressive} \\
\midrule
Prediction & Higher mean ordinary text-token log likelihood & Higher mean raw full-vocabulary token log likelihood \\
Candidate scoring & Teacher-forced text with supplied candidate speech & Teacher-forced speech units (S$\to$S) or text tokens (S$\to$T) \\
Sampling / decoding temperature & Not used & Not used \\
Boundary policy & Rank 1; retry both candidates at rank 3 if either exhausts speech & Native token sequence; no rank fallback \\
Audio frame padding & 80 ms after end VAD & 40 ms after the same end-VAD cutoff \\
Evaluation size & 1,871 stories for each of sSC and tSC & 1,871 stories for each task and direction \\
\bottomrule
\end{tabularx}
\caption{Central likelihood-evaluation settings for StoryCloze. Both candidates are scored independently. Our current accuracy uses all stories, counting remaining incomplete pairs as incorrect. The rank-3 fallback policy was selected after inspecting failures on this dataset. SpiritLM S$\to$T conditions on prompt speech only; our evaluator additionally consumes candidate speech, so their conditioning protocols differ.}
\label{tab:story-cloze-evaluation-settings}
\end{table*}


==> gemini_emo.tex <==
% Requires \usepackage{booktabs}
\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Model & Happy & Sad & Angry & Overall \\
\midrule
Original prefix only & 64.6 & 92.7 & 77.1 & 78.1 \\
\midrule
Speech-only (80k) & 66.9 & 91.0 & 65.0 & 74.3 \\
Ours ($\lambda=0$, 100k) & 66.5 & 88.5 & 69.2 & 74.7 \\
Ours ($\lambda=0.5$, 100k) & 68.3 & 88.8 & 67.3 & 74.8 \\
MiMo-Audio Base & 74.8 & 64.8 & 48.8 & 62.8 \\
SLAM-Large & 69.4 & 30.8 & 1.5 & 33.9 \\
Llama-Mimi 1.3B & 59.6 & 89.6 & 55.0 & 68.1 \\
Llama-Mimi 8B & 62.9 & 91.7 & 60.8 & 71.8 \\
SpiritLM Base & 78.5 & 20.2 & 3.1 & 34.0 \\
SpiritLM Expressive & 77.3 & 79.0 & 8.3 & 54.9 \\
\bottomrule
\end{tabular}
\caption{Gemini-Emo three-way accuracy (\%; higher is better), using argmax over happy, sad, and angry from emotion2vec+. Neutral prompts are excluded. The original-prefix reference evaluates 96 prefixes per emotion once each. Model rows evaluate jointly synthesized prompt-plus-continuation waveforms from the full-floor rerun, with five samples per prefix (480 attempts per emotion). Overall is the macro average of the three emotion accuracies. Failed or empty generations count as misses.}
\label{tab:gemini-emo-full-floor-three-way}
\end{table}


==> gemini_emo_prompts.tex <==
% Requires \usepackage{booktabs,tabularx}
% Exact prompt templates are reconstructed from gemini_emo/texts.json and
% gemini_emo/raw/item_01/{happy,sad,angry}.json.
\begin{table*}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\textwidth}{@{}p{0.17\textwidth}p{0.22\textwidth}X@{}}
\toprule
\textbf{Prompt purpose} & \textbf{Model} & \textbf{Prompt template} \\
\midrule
Text generation
  & \texttt{gemini-3.7-flash}
  & \parbox[t]{\linewidth}{Create exactly 25 English speech-continuation stimulus items. For every item: write one shared prefix of 7--12 words as a natural, affect-neutral, syntactically unfinished conversational turn; write emotion-specific 5--14-word suffixes that complete that prefix; form each carrier as \texttt{PREFIX + `` '' + SUFFIX}; use varied, ordinary ASR-friendly language; and return the supplied item schema. The generation ran in batches through 500 items.} \\
\midrule
Shared TTS interface
  & \parbox[t]{\linewidth}{\texttt{gemini-3.1-flash-}\par\texttt{tts-preview}\\voice: \texttt{Schedar}}
  & \parbox[t]{\linewidth}{Synthesize speech for the transcript below.\par\medskip\textbf{AUDIO PROFILE:} Use one consistent adult speaker identity and a standard American English accent.\par\medskip\textbf{SCENE:} This is a natural conversation with one familiar listener in a quiet room.\par\medskip\textbf{DIRECTOR'S NOTES:} \texttt{<EMOTION-SPECIFIC DIRECTOR'S NOTES>}\par\medskip Speak the transcript exactly once and verbatim. Do not read these directions. Do not add, remove, or replace words. Do not laugh, cry, sigh, gasp, whisper, shout, or add nonverbal sounds.\par\medskip\textbf{TRANSCRIPT:} \texttt{<TRANSCRIPT>}} \\
  \midrule
Happy director's notes
  &
  & \parbox[t]{\linewidth}{Convey a small, private happiness, as if sharing good news with someone you trust. Keep an easy moderate pace and soft-to-medium energy. Let a subtle smile warm the tone and add light upward inflections. Sound understated but unmistakably pleased, not breathy, cute, or theatrical. Apply these cues from the first word, including the neutral lead-in. Keep the performance conversational, coherent, and moderately expressive rather than exaggerated.} \\
Sad director's notes
  &
  & \parbox[t]{\linewidth}{Convey strong genuine sorrow while trying to remain composed. Use a soft voice, slow measured pacing, lowered resonance, and pronounced downward intonation. Sound deeply sad but never cry, sob, or become theatrical. Apply these cues from the first word, including the neutral lead-in. Keep the performance conversational, coherent, and moderately expressive rather than exaggerated.} \\
Angry director's notes
  & 
  & \parbox[t]{\linewidth}{Sound clearly angry but fully controlled. Use a firm tense tone, clipped articulation, strong stress, deliberate pacing, and moderately high energy. Address the listener directly without shouting. Apply these cues from the first word, including the neutral lead-in. Keep the performance conversational, coherent, and moderately expressive rather than exaggerated.} \\
\bottomrule
\end{tabularx}
\caption{Gemini-Emo language-model and TTS prompt specification. The shared TTS row applies to all three emotion prompts. Each prompt inserts one emotion-specific director instruction between the scene and transcript sections. }
\label{tab:gemini-emo-prompt-templates}

\end{table*}


==> gemini_emo_report_with_cont.tex <==
% Requires:
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{array}
% \usepackage[table]{xcolor}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}

% First line: full prompt + continuation
% Second line (gray): continuation only
\newcommand{\gemoCell}[4]{%
  \begin{tabular}{@{}c@{}}
    $#1 \pm #2$ \\
    \textcolor{black!65}{$#3 \pm #4$}
  \end{tabular}%
}

\newcommand{\gemoRef}[2]{%
  \begin{tabular}{@{}c@{}}
    $#1 \pm #2$ \\
    \textcolor{black!65}{--}
  \end{tabular}%
}

\caption{
Gemini-Emo three-way emotion classification accuracy (\%, higher is better) using
emotion2vec-plus-large~\cite{ma2024emotion2vec}.
Each cell reports full prompt-plus-continuation accuracy on the first line and
continuation-only accuracy on the second line in gray. We compute 95\% percentile bootstrap confidence intervals using 10,000 resamples of the 96 triplets, retaining all five generated samples for each emotion within a resampled triplet.
Overall is the macro average over happy, sad, and angry.
The original-prefix reference is evaluated only on the speech prompt.
Empty generations are counted as incorrect.
}
\label{tab:gemini-emo-full-and-continuation-three-way}
\label{tab:gemini-emo-full-floor-three-way}
\label{tab:gemini-emo-continuation-only-three-way}

\begin{tabularx}{\textwidth}{
@{}
>{\raggedright\arraybackslash}X
c
c
c
c
@{}
}
\toprule
\textbf{Model}
& \textbf{Happy}
& \textbf{Sad}
& \textbf{Angry}
& \textbf{Overall} \\
\midrule

% ---------------------------------------------------------------
\rowcolor{gray!12}
\textbf{Original prefix only}
    & \gemoRef{64.6}{9.4}
    & \gemoRef{92.7}{4.7}
    & \gemoRef{77.1}{8.3}
    & \gemoRef{78.1}{4.3} \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{blue!18}
\multicolumn{5}{@{}l}{\textbf{Our models}} \\

Speech-only
    & \gemoCell{66.9}{6.1}{54.2}{5.2}
    & \gemoCell{91.0}{3.7}{76.9}{4.3}
    & \gemoCell{65.0}{6.1}{36.7}{4.5}
    & \gemoCell{74.3}{2.8}{55.9}{2.7} \\

\rowcolor{blue!4}
\textbf{TGSLM} ($\lambda=0$)
    & \gemoCell{66.5}{6.0}{57.7}{4.9}
    & \gemoCell{88.5}{4.4}{72.1}{4.6}
    & \gemoCell{69.2}{6.0}{43.3}{5.0}
    & \gemoCell{74.7}{3.2}{57.7}{2.8} \\

\rowcolor{blue!7}
\textbf{TGSLM-distill} ($\lambda=0.5$)
    & \gemoCell{68.3}{5.9}{60.0}{4.4}
    & \gemoCell{88.8}{3.9}{77.3}{4.3}
    & \gemoCell{67.3}{5.3}{34.8}{4.7}
    & \gemoCell{74.8}{2.7}{57.4}{2.6} \\

\rowcolor{blue!12}
\textbf{TGSLM-Large-distill} ($\lambda=0.5$)
    & \gemoCell{66.5}{5.4}{54.8}{5.1}
    & \gemoCell{91.7}{3.3}{80.4}{4.3}
    & \gemoCell{62.3}{5.7}{38.5}{4.4}
    & \gemoCell{73.5}{2.7}{57.9}{2.6} \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{green!12}
\multicolumn{5}{@{}l}{
    \textbf{\textcolor{green!40!black}{External models with full acoustic information}}
} \\

MiMo-Audio Base
    & \gemoCell{74.8}{5.0}{73.1}{4.2}
    & \gemoCell{64.8}{5.8}{45.8}{5.2}
    & \gemoCell{48.8}{5.7}{25.6}{4.6}
    & \gemoCell{62.8}{3.2}{48.2}{2.5} \\

Llama-Mimi 1.3B
    & \gemoCell{59.6}{5.8}{46.5}{4.9}
    & \gemoCell{89.6}{4.0}{87.7}{4.0}
    & \gemoCell{55.0}{6.1}{45.0}{4.8}
    & \gemoCell{68.1}{2.9}{59.7}{2.3} \\

Llama-Mimi 8B
    & \gemoCell{62.9}{5.7}{46.0}{4.8}
    & \gemoCell{91.7}{3.1}{88.5}{3.2}
    & \gemoCell{60.8}{5.8}{46.5}{5.0}
    & \gemoCell{71.8}{2.6}{60.3}{2.3} \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{orange!12}
\multicolumn{5}{@{}l}{
    \textbf{\textcolor{orange!55!black}{External models without full acoustic information}}
} \\

SLAM-Large
    & \gemoCell{69.4}{5.6}{65.4}{4.2}
    & \gemoCell{30.8}{5.2}{34.4}{4.6}
    & \gemoCell{1.5}{1.1}{1.9}{1.1}
    & \gemoCell{33.9}{1.9}{33.9}{1.9} \\

SpiritLM Base
    & \gemoCell{78.5}{4.8}{75.4}{4.4}
    & \gemoCell{20.2}{4.3}{23.8}{4.3}
    & \gemoCell{3.1}{1.8}{2.7}{1.6}
    & \gemoCell{34.0}{1.7}{34.0}{1.8} \\

SpiritLM Expressive
    & \gemoCell{77.3}{5.5}{66.0}{4.9}
    & \gemoCell{79.0}{5.2}{76.7}{4.0}
    & \gemoCell{8.3}{3.3}{9.2}{2.9}
    & \gemoCell{54.9}{2.7}{50.6}{2.2} \\

\bottomrule
\end{tabularx}

\vspace{1mm}
\end{table*}

==> genppl.tex <==
% Requires:
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{array}
% \usepackage[table]{xcolor}

% Ground-truth speaker: artifacts/emilia_ground_truth_speaker_20260921/summary.json (genppl_min_k)
% Ground-truth OLMo: artifacts/emilia_ground_truth_genppl_20260921_v2/summary.json (genppl_min_k)
% Source: artifacts/qwen3_1p7b_665k_eval_20260921/emilia/min_k/summary.csv
% Quality: artifacts/qwen3_1p7b_665k_eval_20260921/emilia/quality_summary.json
% Ground-truth UTMOS: artifacts/qwen3_1p7b_665k_eval_20260921/summary.json (ground_truth.genppl_min_k)
% Current 26-condition min-k aggregation; scores rounded directly from full precision.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.06}

\caption{
Generation-based metrics on the Emilia test set, including genPPL, speaker similarity
(Spk. sim.), and UTMOS-v2~\cite{baba2024utmosv2}; see Sec.~\ref{sec:eval} for details.
For the Whisper prompt transcript, we use Whisper \texttt{small.en} to transcribe the speech prompt and condition generation on the resulting text.
All rows are evaluated on the intersection of prompts with non-empty continuations,
resulting in 1,406 of 1,500 prompts with at least one continuation and 6,022 of 7,500 continuations.
\textbf{TGSLM-Large-distill} uses a distillation weight of $\lambda=0.5$ and text replay.
}
\label{tab:genppl}

\begin{tabularx}{\linewidth}{
@{}
>{\raggedright\arraybackslash}X
>{\centering\arraybackslash}p{0.145\linewidth}
>{\centering\arraybackslash}p{0.065\linewidth}
>{\centering\arraybackslash}p{0.085\linewidth}
r
r
r
@{}
}
\toprule
\textbf{Model}
& \textbf{Direction}
& \textbf{Params}
& \textbf{Data}
& \textbf{GenPPL $\downarrow$}
& \textbf{Spk. sim. $\uparrow$}
& \textbf{UTMOS $\uparrow$} \\
\midrule

% ---------------------------------------------------------------
\rowcolor{gray!10}
\textbf{Ground truth}
    & --
    & --
    & --
    & 44.6
    & 0.73
    & 2.81 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
% Use a normal 7-cell row so the color width exactly matches result rows.
\rowcolor{gray!15}
\multicolumn{7}{@{}l@{}}{
    \textbf{Speech-only baselines (no text guidance)}
} \\

Speech-only
    & S $\rightarrow$ S
    & 0.8B
    & 21.3k h
    & 146.4
    & 0.41
    & 2.54 \\

Interleaved
    & S $\rightarrow$ S
    & 0.8B
    & 21.3k h
    & 156.3
    & 0.36
    & 2.35 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{blue!18}
\makebox[0pt][l]{\textbf{TGSLM variants}}
    & & & & & & \\

%\rowcolor{blue!4}
TGSLM
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 57.4
    & 0.36
    & 2.40 \\

%\rowcolor{blue!4}
\quad + self-generated prompt text
    & (S, T) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 60.3
    & 0.38
    & 2.40 \\

%\rowcolor{blue!4}
\quad + distillation ($\lambda=0.25$)
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 54.4
    & 0.36
    & 2.40 \\


\quad + distillation + text replay
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 49.5
    & 0.37
    & 2.44 \\


TGSLM-Large-distill
    & S $\rightarrow$ (T, S)
    & 1.9B
    & 135k h
    & 44.6
    & 0.42
    & 2.63 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{orange!18}
\makebox[0pt][l]{\textbf{Text-leading references}}
    & & & & & & \\

Oracle prompt text
    & (T, S) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 39.6
    & 0.41
    & 2.49 \\

Whisper prompt transcript
    & (T, S) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 56.6
    & 0.41
    & 2.49 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{gray!15}
\makebox[0pt][l]{\textbf{External models}}
    & & & & & & \\

\rowcolor{orange!8}
\makebox[0pt][l]{%
    \textbf{\textcolor{orange!55!black}{With limited acoustic information}}%
}
    & & & & & & \\

SpiritLM Base
    & S $\rightarrow$ S
    & 7B
    & 570k h
    & 30.0
    & 0.05
    & 2.39 \\

SpiritLM Expressive
    & S $\rightarrow$ S
    & 7B
    & 570k h
    & 65.4
    & 0.07
    & 2.45 \\

SLAM-Large
    & S $\rightarrow$ S
    & 1.3B
    & 81.0k h
    & 53.3
    & 0.06
    & 3.46 \\

\addlinespace[1pt]

\rowcolor{green!8}
\makebox[0pt][l]{%
    \textbf{\textcolor{green!40!black}{With richer acoustic information}}%
}
    & & & & & & \\

MiMo-Audio-7B-Base
    & S $\rightarrow$ (T, S)
    & 7B
    & \mbox{$>$100M h}
    & 14.6
    & 0.40
    & 3.03 \\

Llama-Mimi-1.3B
    & S $\rightarrow$ S
    & 1.3B
    & 240k h
    & 86.1
    & 0.39
    & 2.60 \\

Llama-Mimi-8B
    & S $\rightarrow$ S
    & 8B
    & 240k h
    & 52.0
    & 0.41
    & 2.59 \\

\bottomrule
\end{tabularx}

\vspace{1mm}
\end{table}


==> genppl_new.tex <==
% Requires:
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{array}
% \usepackage[table]{xcolor}

% Ground-truth speaker: artifacts/emilia_ground_truth_speaker_20260921/summary.json (genppl_min_k)
% Ground-truth OLMo: artifacts/emilia_ground_truth_genppl_20260921_v2/summary.json (genppl_min_k)
% Source: artifacts/qwen3_1p7b_665k_eval_20260921/emilia/min_k/summary.csv
% Quality: artifacts/qwen3_1p7b_665k_eval_20260921/emilia/quality_summary.json
% Ground-truth UTMOS: artifacts/qwen3_1p7b_665k_eval_20260921/summary.json (ground_truth.genppl_min_k)
% Current 26-condition min-k aggregation; scores rounded directly from full precision.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.06}

\caption{
Generation-based metrics on the Emilia test set, including genPPL, auto-BLEU with bi-gram (BLEU), speaker similarity
(Spk), and UTMOS-v2 (UTMOS)~\citep{baba2024utmosv2}; see Sec.~\ref{sec:eval} for details.
For the Whisper prompt transcript, we use Whisper \texttt{small.en} to transcribe the speech prompt and condition generation on the resulting text.
All rows are evaluated on the intersection of prompts with non-empty continuations,
resulting in 1,406 of 1,500 prompts with at least one continuation and 6,022 of 7,500 continuations.
\textbf{TGSLM-Large-distill} uses a distillation weight of $\lambda=0.5$ and text replay.
}
\label{tab:genppl}

\begin{tabularx}{\linewidth}{
@{}
>{\raggedright\arraybackslash}X
>{\centering\arraybackslash}p{0.145\linewidth}
>{\centering\arraybackslash}p{0.065\linewidth}
>{\centering\arraybackslash}p{0.085\linewidth}
r
r
r
r
@{}
}
\toprule
\textbf{Model}
& \textbf{Direction}
& \textbf{Params}
& \textbf{Data}
& \textbf{GenPPL $\downarrow$}
& \textbf{BLEU$\downarrow$}
& \textbf{Spk  $\uparrow$}
& \textbf{UTMOS $\uparrow$} \\
\midrule

% ---------------------------------------------------------------
\rowcolor{gray!10}
\textbf{Ground truth}
    & --
    & --
    & --
    & 44.6
    & 5.9
    & 0.73
    & 2.81 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
% Use a normal 8-cell row so the color width exactly matches result rows.
\rowcolor{gray!15}
\multicolumn{8}{@{}l@{}}{
    \textbf{Speech-only baselines (no text guidance)}
} \\

Speech-only
    & S $\rightarrow$ S
    & 0.8B
    & 21.3k h
    & 146.4
    & 4.3
    & 0.41
    & 2.54 \\

Interleaved
    & S $\rightarrow$ S
    & 0.8B
    & 21.3k h
    & 156.3
    & 5.5
    & 0.36
    & 2.35 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{blue!18}
\makebox[0pt][l]{\textbf{TGSLM variants}}
    & & & & & & & \\

%\rowcolor{blue!4}
TGSLM
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 57.4
    & 3.9
    & 0.36
    & 2.40 \\

%\rowcolor{blue!4}
\quad + self-generated prompt text
    & (S, T) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 60.3
    & 3.8
    & 0.38
    & 2.40 \\

%\rowcolor{blue!4}
\quad + distillation ($\lambda=0.25$)
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 54.4
    & 4.4
    & 0.36
    & 2.40 \\


\quad + distillation + text replay
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 49.5
    & 5.0
    & 0.37
    & 2.44 \\


TGSLM-Large-distill
    & S $\rightarrow$ (T, S)
    & 1.9B
    & 135k h
    & 44.6
    & 5.4
    & 0.42
    & 2.63 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{orange!18}
\makebox[0pt][l]{\textbf{Text-leading references}}
    & & & & & & & \\

Oracle prompt text
    & (T, S) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 39.6
    & 5.3
    & 0.41
    & 2.49 \\

Whisper prompt transcript
    & (T, S) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 56.6
    & 6.5
    & 0.41
    & 2.49 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{gray!15}
\makebox[0pt][l]{\textbf{External models}}
    & & & & & & & \\

\rowcolor{orange!8}
\multicolumn{8}{@{}l@{}}{
    \textbf{\textcolor{orange!55!black}{With limited acoustic information}}%
} \\
%    & & & & & & & \\

SpiritLM Base
    & S $\rightarrow$ S
    & 7B
    & 570k h
    & 30.0
    & 13.3
    & 0.05
    & 2.39 \\

SpiritLM Expressive
    & S $\rightarrow$ S
    & 7B
    & 570k h
    & 65.4
    & 8.9
    & 0.07
    & 2.45 \\

SLAM-Large
    & S $\rightarrow$ S
    & 1.3B
    & 81.0k h
    & 53.3
    & 10.1
    & 0.06
    & 3.46 \\

\addlinespace[1pt]

\rowcolor{green!8}
\multicolumn{8}{@{}l@{}}{
    \textbf{\textcolor{green!40!black}{With richer acoustic information}}%
} \\
% \multicolumn{8}{@{}l@{}}{
%     \textbf{Speech-only baselines (no text guidance)}
% }
%     & & & & & & & \\

MiMo-Audio-7B-Base
    & S $\rightarrow$ (T, S)
    & 7B
    & \mbox{$>$100M h}
    & 14.6
    & 20.8
    & 0.40
    & 3.03 \\

Llama-Mimi-1.3B
    & S $\rightarrow$ S
    & 1.3B
    & 240k h
    & 86.1
    & 6.2
    & 0.39
    & 2.60 \\

Llama-Mimi-8B
    & S $\rightarrow$ S
    & 8B
    & 240k h
    & 52.0
    & 7.0
    & 0.41
    & 2.59 \\

\bottomrule
\end{tabularx}

\vspace{1mm}
\end{table}


==> genppl_v2.tex <==
% Requires:
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{array}
% \usepackage[table]{xcolor}

% Nine-condition aggregation: /share/data/speech-lang/users/jjery2243542/continuous_gslm/cache/artifacts/emilia_internal9_min_k_20260923/summary.json
% Selection: /share/data/speech-lang/users/jjery2243542/continuous_gslm/cache/artifacts/emilia_internal9_min_k_20260923/selected_samples.tsv
% Source scores reused; genPPL one decimal, speaker cosine and UTMOS two decimals.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.06}

\caption{
Generation-based metrics on the Emilia test set, including genPPL, speaker similarity
(Spk. sim.), and UTMOS-v2~\cite{baba2024utmosv2}; see Sec.~\ref{sec:eval} for details.
For the Whisper prompt transcript, we use Whisper \texttt{small.en} to transcribe the speech prompt and condition generation on the resulting text.
All rows are evaluated on the intersection of prompts with non-empty continuations,
resulting in 1433 of 1473 prompts with at least one continuation and 6702 of 7365 continuations.
\textbf{TGSLM-Large-distill} uses a distillation weight of $\lambda=0.5$ and text replay.
}
\label{tab:genppl}

\begin{tabularx}{\linewidth}{
@{}
>{\raggedright\arraybackslash}X
>{\centering\arraybackslash}p{0.145\linewidth}
>{\centering\arraybackslash}p{0.065\linewidth}
>{\centering\arraybackslash}p{0.085\linewidth}
r
r
r
@{}
}
\toprule
\textbf{Model}
& \textbf{Direction}
& \textbf{Params}
& \textbf{Data}
& \textbf{GenPPL $\downarrow$}
& \textbf{Spk. sim. $\uparrow$}
& \textbf{UTMOS $\uparrow$} \\
\midrule

% ---------------------------------------------------------------
\rowcolor{gray!10}
\textbf{Ground truth}
    & --
    & --
    & --
    & 45.0
    & 0.73
    & 2.80 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
% Use a normal 7-cell row so the color width exactly matches result rows.
\rowcolor{gray!20}
\multicolumn{7}{@{}l@{}}{
    \textbf{Speech-only baselines (no text guidance)}
} \\
%    & & & & & & \\

Speech-only
    & S $\rightarrow$ S
    & 0.8B
    & 21.3k h
    & 146.8
    & 0.41
    & 2.54 \\

Interleaved
    & S $\rightarrow$ S
    & 0.8B
    & 21.3k h
    & 156.4
    & 0.36
    & 2.35 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{blue!18}
\makebox[0pt][l]{\textbf{TGSLM variants}}
    & & & & & & \\

\rowcolor{blue!4}
\textbf{TGSLM}
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 58.1
    & 0.35
    & 2.39 \\

\rowcolor{blue!4}
\quad \textbf{+ self-generated prompt text}
    & (S, T) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 60.7
    & 0.37
    & 2.39 \\

\rowcolor{blue!4}
\quad \textbf{+ distillation} ($\lambda=0.25$)
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 54.8
    & 0.36
    & 2.40 \\

\rowcolor{blue!4}
\quad \textbf{+ distillation + text replay}
    & S $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 50.0
    & 0.37
    & 2.43 \\

\rowcolor{blue!12}
\textbf{TGSLM-Large-distill}
    & S $\rightarrow$ (T, S)
    & 1.9B
    & 135k h
    & \textbf{45.0}
    & \textbf{0.42}
    & \textbf{2.62} \\

\addlinespace[2pt]

% ---------------------------------------------------------------
\rowcolor{orange!18}
\makebox[0pt][l]{\textbf{Text-leading references}}
    & & & & & & \\

Oracle prompt text
    & (T, S) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 39.9
    & 0.41
    & 2.49 \\

Whisper prompt transcript
    & (T, S) $\rightarrow$ (T, S)
    & 0.8B
    & 21.3k h
    & 57.7
    & 0.40
    & 2.48 \\

\addlinespace[2pt]

% ---------------------------------------------------------------
% Commented external rows retain historical 26-condition values and are excluded here.
% \rowcolor{gray!15}
% \makebox[0pt][l]{\textbf{External models}}
%     & & & & & & \\

% \rowcolor{orange!8}
% \makebox[0pt][l]{%
%     \textbf{\textcolor{orange!55!black}{With limited acoustic information}}%
% }
%     & & & & & & \\

% SpiritLM Base
%     & S $\rightarrow$ S
%     & 7B
%     & 570k h
%     & 30.0
%     & 0.05
%     & 2.39 \\

% SpiritLM Expressive
%     & S $\rightarrow$ S
%     & 7B
%     & 570k h
%     & 65.4
%     & 0.07
%     & 2.45 \\

% SLAM-Large
%     & S $\rightarrow$ S
%     & 1.3B
%     & 81.0k h
%     & 53.3
%     & 0.06
%     & 3.46 \\

% \addlinespace[1pt]

% \rowcolor{green!8}
% \makebox[0pt][l]{%
%     \textbf{\textcolor{green!40!black}{With richer acoustic information}}%
% }
%     & & & & & & \\

% MiMo-Audio-7B-Base
%     & S $\rightarrow$ (T, S)
%     & 7B
%     & \mbox{$>$100M h}
%     & 14.6
%     & 0.40
%     & 3.03 \\

% Llama-Mimi-1.3B
%     & S $\rightarrow$ S
%     & 1.3B
%     & 240k h
%     & 86.1
%     & 0.39
%     & 2.60 \\

% Llama-Mimi-8B
%     & S $\rightarrow$ S
%     & 8B
%     & 240k h
%     & 52.0
%     & 0.41
%     & 2.59 \\

\bottomrule
\end{tabularx}

\vspace{1mm}
\end{table}



==> genppl_w_bleu.tex <==
% Ground-truth speaker: artifacts/emilia_ground_truth_speaker_20260921/summary.json (genppl_min_k)
% Requires booktabs and tabularx in the document preamble.
% Ground-truth OLMo: artifacts/emilia_ground_truth_genppl_20260921_v2/summary.json (genppl_min_k)
% Source: artifacts/qwen3_1p7b_665k_eval_20260921/emilia/min_k/summary.csv
% Quality: artifacts/qwen3_1p7b_665k_eval_20260921/emilia/quality_summary.json
% Ground-truth UTMOS: artifacts/qwen3_1p7b_665k_eval_20260921/summary.json (ground_truth.genppl_min_k)
% Current 27-condition aggregation: /share/data/speech-lang/users/jjery2243542/continuous_gslm/cache/artifacts/emilia_legacy_openelm27_20260924/summary.json
% Original 26-condition source files remain unchanged.
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{2.5pt}

\caption{GenPPL, speaker similarity, UTMOS-v2, and Auto-BLEU$_2$ on the Emilia test set using the shared min-$k$ selection
across all 27 evaluated model/direction conditions, including the scaled model.
For each prompt, $k$ is the minimum number of valid continuations across conditions;
we retain each condition's first $k$ valid samples in sample order.
This yields 1,396 shared prompts and 5,863 continuations per condition.
GenPPL is computed from pooled token losses.
S and T denote speech and text, respectively.
Speech continuations are transcribed with Whisper \texttt{small.en}
before scoring with OLMo-3-7B.
Speaker similarity is WavLM-large/ECAPA cosine against the original prompt crop,
reported on its original cosine scale; UTMOS-v2 scores generated continuations only.
Quality means use valid metric scores within the same min-$k$ selection. Auto-BLEU$_2$ is the arithmetic mean of repeated-bigram-occurrence ratios on full utterances (prompt plus continuation), on a 0--1 scale. It uses saved joint-waveform ASR for speech-input/speech-output rows and the existing prompt-plus-output text for other directions, before genPPL prompt removal. Words are lowercased with ASCII punctuation removed. Ground-truth Auto-BLEU$_2$ uses full aligned reference text weighted by $k$.
Ground-truth UTMOS-v2 uses full original recordings, weighted by each prompt's $k$.
Ground-truth speaker similarity compares the original continuation with its prompt crop, using the same $k$ weights.
Dashes indicate unmeasured or inapplicable metrics; T $\rightarrow$ S UTMOS-v2 and external T $\rightarrow$ S speaker similarity have not been evaluated. Interleaved T $\rightarrow$ S speaker similarity uses the original reference despite text-only conditioning.
The previous OpenELM model uses its saved historical genPPL and generations with oracle prompt text, silence penalty 3, and text repetition penalty 1.5; its speaker and UTMOS-v2 scores are newly measured. Ground-truth perplexity scores the aligned continuation with prompt tokens excluded from loss, using the same $k$ weights.}
\label{tab:genppl}

\begin{tabularx}{\linewidth}{
@{}
>{\raggedright\arraybackslash}X
l
r
r
r
r
r
r
@{}
}
\toprule
\textbf{Model}
& \textbf{Direction}
& \textbf{Params}
& \textbf{Speech data}
& \textbf{GenPPL $\downarrow$}
& \textbf{Spk. sim. $\uparrow$}
& \textbf{UTMOS-v2 $\uparrow$}
& \textbf{Auto-BLEU$_2$ $\downarrow$} \\
\midrule

Speech-only
    & S $\rightarrow$ S
    & 0.8B & 21.3k h
    & 146.5 & 0.41 & 2.54 & 0.043 \\
\midrule

Interleaved
    & S $\rightarrow$ S
    & 0.8B & 21.3k h
    & 157.1 & 0.36 & 2.35 & 0.055 \\
    & S $\rightarrow$ T
    & & & 42.9 & -- & -- & 0.054 \\
    & T $\rightarrow$ S
    & & & 201.7 & 0.08 & -- & 0.033 \\
    & T $\rightarrow$ T
    & & & 27.7 & -- & -- & 0.122 \\
\midrule

TGSLM
    & S $\rightarrow$ (T, S)
    & 0.8B & 21.3k h
    & 57.4 & 0.36 & 2.40 & 0.039 \\

+ self-generated transcription
    & (S, $\hat{T}$) $\rightarrow$ (T, S)
    & 0.8B & 21.3k h
    & 60.2 & 0.38 & 2.40 & 0.038 \\

+ distillation ($\lambda=0.25$)
    & S $\rightarrow$ (T, S)
    & 0.8B & 21.3k h
    & 54.4 & 0.36 & 2.40 & 0.044 \\

+ distillation + text replay
    & S $\rightarrow$ (T, S)
    & 0.8B & 21.3k h
    & 49.6 & 0.37 & 2.44 & 0.049 \\
\midrule

TGSLM-large + distillation ($\lambda=0.5$) + text replay
    & S $\rightarrow$ (T, S)
    & 1.9B & 135k h
    & 44.7 & 0.42 & 2.63 & 0.054 \\
\midrule

Text-leading with oracle prompt text
    & (T, S) $\rightarrow$ (T, S)
    & 0.8B & 21.3k h
    & 39.6 & 0.41 & 2.49 & 0.053 \\

Text-leading with Whisper small.en transcription
    & ($\hat{T}$, S) $\rightarrow$ (T, S)
    & 0.8B & 21.3k h
    & 56.4 & 0.41 & 2.49 & 0.065 \\

\midrule
Previous model (OpenELM-270M backbone)
    & (T, S) $\rightarrow$ (T, S)
    & -- & 10k h
    & 52.9 & 0.34 & 2.48 & 0.065 \\
\midrule

\multicolumn{8}{l}{\textit{External models}} \\
\midrule

SpiritLM Base
    & S $\rightarrow$ S
    & 7B & 570k h
    & 30.0 & 0.05 & 2.39 & 0.133 \\
    & S $\rightarrow$ T
    & & & 15.7 & -- & -- & 0.138 \\
    & T $\rightarrow$ S
    & & & 27.6 & -- & -- & 0.132 \\
    & T $\rightarrow$ T
    & & & 11.0 & -- & -- & 0.170 \\

SpiritLM Expressive
    & S $\rightarrow$ S
    & 7B & 570k h
    & 65.6 & 0.07 & 2.45 & 0.089 \\
    & S $\rightarrow$ T
    & & & 16.2 & -- & -- & 0.147 \\
    & T $\rightarrow$ S
    & & & 59.8 & -- & -- & 0.083 \\
    & T $\rightarrow$ T
    & & & 11.2 & -- & -- & 0.167 \\

MiMo-Audio-7B-Base
    & S $\rightarrow$ (T, S)
    & 7B & $>$100M h
    & 14.6 & 0.40 & 3.03 & 0.206 \\

SLAM-Large
    & S $\rightarrow$ S
    & 1.3B & 81.0k h
    & 53.2 & 0.06 & 3.46 & 0.101 \\

Llama-Mimi-1.3B
    & S $\rightarrow$ S
    & 1.3B & 240k h
    & 86.3 & 0.39 & 2.60 & 0.062 \\

Llama-Mimi-8B
    & S $\rightarrow$ S
    & 8B & 240k h
    & 52.2 & 0.41 & 2.59 & 0.070 \\

\midrule
Ground truth (aligned text / full audio)
    & -- & -- & -- & 44.4 & 0.74 & 2.81 & 0.059 \\

\bottomrule
\end{tabularx}

\vspace{1mm}
\end{table}


==> procon.tex <==
\begin{table}[t]
\centering
\caption{
Comparison of how text is used at inference in speech-text language models. \textbf{Speech-only prompt} indicates whether inference can begin from speech without using its transcription. \textbf{Text-guided speech generation} indicates whether generated text explicitly conditions the subsequent speech generation.
}
\label{tab:text_usage}
\begin{tabular}{lccc}
\toprule
Model  & Speech-only prompt& Text-guided speech generation \\
\midrule
Inner monologue  & \xmark & \checkmark \\
Interleaved      & \checkmark     & \xmark \\
TGSLM             & \checkmark     & \checkmark \\
\bottomrule
\end{tabular}
\end{table}

==> training_hyperparameters.tex <==
% Requires \usepackage{booktabs,tabularx}
% Verified against saved training conf.yaml files, not only launcher defaults.
% Exact source paths, hashes, and extracted values: training_hyperparameters.sources.json
% Scaled run refers to the 665k-step Qwen3-1.7B production recipe.
% Additional tables below give recorded decoding settings and external checkpoints.
% Their provenance is recorded under decoding_sources in the companion JSON.
\begin{table}[h]
\centering
\footnotesize
\begingroup
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{\textwidth}{@{}p{0.27\textwidth}*{3}{>{\raggedright\arraybackslash}X}@{}}
\toprule
\textbf{Hyperparameter} & \textbf{Architecture ablations} & \textbf{Distillation ablations} & \textbf{TGSLM-large} \\
\midrule
\multicolumn{4}{@{}l}{\textit{Training}} \\
\midrule
Backbone & Qwen3-0.6B-Base & Qwen3-0.6B-Base & Qwen3-1.7B-Base \\
Optimizer updates & 40,000; 50,000 for model with text replay & 100,000 & 665,000 \\
Audio budget (s/GPU/update) & 480 & 540 & 240 \\
GPUs & 4 & 4 & 4 \\
%Gradient accumulation & 1 & 1 & 1 \\
Peak learning rate & $5\times10^{-4}$ & $5\times10^{-4}$ & $3\times10^{-4}$ \\
Warmup updates & 5,000 & 5,000 & 5,000 \\
Final / peak learning rate ratio & 0.1 & 0.1 & 0.1 \\
Bucket bin duration (s) & 2 & 2 & 2 \\ 
\midrule
FineWeb replay probability & 0; 0.2 for replay-enabled model & 0.2 & 0.2 \\
Replay tokens/GPU/update & 2,048  & 2,048 & 2,048 \\
%PLAN KL weight $\lambda$ & 0; 0.25 for F and G & $0$, $0.1$, $0.25$, $0.5$, $0.75$ & 0.5 \\
%KL temperature $T$ & 1 (F and G) & 1; also 2 and 3 at $\lambda=0.5$ & 1 \\
\midrule
Optimizer & \multicolumn{3}{l}{AdamW8bit} \\
Adam $(\beta_1,\beta_2)$ & \multicolumn{3}{l}{$(0.9,0.98)$} \\
Adam $\epsilon$ & \multicolumn{3}{l}{$10^{-6}$} \\
Weight decay & \multicolumn{3}{l}{0.01} \\
Learning-rate schedule & \multicolumn{3}{l}{Linear warmup followed by cosine decay} \\
Training precision & \multicolumn{3}{l}{BF16 mixed precision} \\
\midrule
\multicolumn{4}{@{}l}{\textit{Shared decoding settings}} \\
\midrule
Sampling temperature & \multicolumn{3}{l}{0.8 for text, semantic tokens, and flow Gaussian} \\
Nucleus threshold $p$ & \multicolumn{3}{l}{0.95} \\
Flow integration & \multicolumn{3}{l}{Euler, 32 steps} \\
Classifier-free guidance scale & \multicolumn{3}{l}{0.3} \\
Mimi decoder quantizers & \multicolumn{3}{l}{16} \\
%Boundary rank & \multicolumn{3}{l}{1, where serialized boundaries apply} \\
Samples per prompt & \multicolumn{3}{l}{5} \\
%Base seed & \multicolumn{3}{l}{0} \\
Maximum new speech & \multicolumn{3}{l}{10 s (Known-1000); 20 s (Emilia/Gemini-Emo)} \\
%Minimum generated words & \multicolumn{3}{l}{0; 5 for Gemini-Emo generation} \\
%Silence penalization & \multicolumn{3}{l}{Off; weight 10 for the speech-only baseline} \\
\bottomrule
\end{tabularx}
\endgroup
\caption{Training hyperparameters and decoding parameters. }
\label{tab:training-hyperparameters}

\vspace{2pt}
\begin{minipage}{\textwidth}

\end{minipage}
\end{table}

